A Machine Learning Approach to Determine the Semantic Versioning Type of npm Packages Releases

Semantic versioning policy is widely used to indicate the level of changes in a package release. Unfortunately, there are many cases where developers do not respect the semantic versioning policy, leading to the breakage of dependent applications. To reduce such cases, we proposed using machine learning (ML) techniques to effectively predict the new release type, i.e., patch, minor, major, in order to properly determine the semantic versioning type. To perform our prediction, we mined and used a number of features about a release, such as the complexity of the changed code, change types, and development activities. We then used four ML classifiers. To evaluate the performance of the proposed ML classifiers, we conducted an empirical study on 31 JavaScript packages containing a total of approximately 6,260 releases. We started by extracting 41 release level features from historical data of packages' source code and repositories. Then, we used four machine learning classifiers, namely XGBoost, Random Forest, Decision Tree, and Logistic Regression. We found that the XGBoost classifiers performed the best, achieving median ROC AUC values of 0.78, 0.69, and 0.74 for major, minor, and patch releases, respectively. We also found that features related to the change types in a release are the best predictors group of features in determining the semantic versioning type. Finally, we studied the generalizability of determining the semantic versioning type by applying cross-package validation. Our results showed that the general classifier achieved median ROC AUC values of 0.76, 0.69, and 0.75 for major, minor, and patch releases.

==> discussion.tex <==
We may discuss some of the interesting findings, cases, or extra analysis if needed. 


Also, some implication can be discussed here as well.

\rabe{You need an implication/discussion section. }

\rabe{Where does your method mostly fails?}
\rabe{Why are some projects more difficult than others? You can take the two extreme cases license-checker (0.61) vs pacote (0.92).
What about other performance metrics? }

\rabe{Most importantly, how can developers use the features you reported as the most important in deciding the semantic version type?}
\rabe{How can developers deploy your ML pipeline in their own CI to maybe recommend the release type?}

\rabe{You motivate the work by saying that developers often misclassify their semantic version type, how is this work contributing to this problem?}


ALso, relaese on the code review. and integrate our tool in the continouse integration systems.

General \minatiner could use our tool to build a recommendation systems when a developers submit a new version of their package the recommndation tool could flage the use of \sv. Research could replicate our study on other ecosystems.

==> table_feature.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}



